Starlit: Privacy-Preserving Federated Learning to Enhance Financial Fraud Detection

Federated Learning (FL) is a data-minimization approach enabling collaborative model training across diverse clients with local data, avoiding direct data exchange. However, state-of-the-art FL solutions to identify fraudulent financial transactions exhibit a subset of the following limitations. They (1) lack a formal security definition and proof, (2) assume prior freezing of suspicious customers' accounts by financial institutions (limiting the solutions' adoption), (3) scale poorly, involving either $O(n^2)$ computationally expensive modular exponentiation (where $n$ is the total number of financial institutions) or highly inefficient fully homomorphic encryption, (4) assume the parties have already completed the identity alignment phase, hence excluding it from the implementation, performance evaluation, and security analysis, and (5) struggle to resist clients' dropouts. This work introduces Starlit, a novel scalable privacy-preserving FL mechanism that overcomes these limitations. It has various applications, such as enhancing financial fraud detection, mitigating terrorism, and enhancing digital health. We implemented Starlit and conducted a thorough performance analysis using synthetic data from a key player in global financial transactions. The evaluation indicates Starlit's scalability, efficiency, and accuracy.

==> aggregator.tex <==
% !TEX root =Feather.tex
\section{Aggregator}\label{sec:aggregator}

{\bf Not intended for direct use in the whitepaper.} \\
Each bank holds their own data about their customers which looks like
$$ (AccountId, Name, Street, CountryCityZip, Flag).$$
The strings, "Name", "Street", "CountryCityZip" are used to calculate features, see section edit-distance, we will explain how we plan to use the "Flag" to create a feature. \\ 
As explained earlier, to avoid combinatorial explosion, we create a new party, the aggregator, which will be a node in the federated learning model. This aggregator will receive the flags from the banks and combine them in a way that makes the training steps simpler. The process to do this is sketched next.

\begin{enumerate}
    \item SWIFT: For each unique account, $x$, calculate an identifier, $U(x)$, this identifier is strictly one way.
    \item SWIFT: Let $b(x)$ be the bank the account is at, for each bank, $B$, send the following set to $B$, $A_B = \{(U(x), x) | b(x) = B \}$.
    \item SWIFT: Create a (No. transactions x 2) matrix $T$, and send it to the aggregator. Each row of the matrix looks like $(U(x_{i1}), U(x_{i2}))$ where $x_{i1}$ is the OrderingAccount for the $i^{th}$ transaction and $x_{i2}$ is the BeneficiaryAccount.
    \item Bank: Each bank receives $A_B$ and creates $F_B = \{(U(x), F(x)) | x \in  A_B \}$ where $F(x)$ is the "Flag" information associated to $x$. They send $F_B$ to the aggregator.
    \item Aggregator: Receives the matrix $T$, from SWIFT and $F_B$ from each bank, $B$. They then create a new matrix of the same size by replacing $U(x)$ with $F(x)$. This works as $\bigcup_{B} F_B$ only contains one pair with first entry $U(x)$. This matrix is then used as the data for the ML model, if we were not in the federated setting, we would be able to join this matrix to the database SWIFT has along row number. This means there is no need for alignment when training the model.
\end{enumerate}
Assuming all these steps are done in plaintext (with secure sending), the following information is learnt by each party.\\
Bank - learns which of its accounts are in use. \\
Aggregator -  learns which $U(x)$ come from each bank. It can use this information to calculate how many transactions are between each pair of banks, it can also calculate how many transactions between each pair of $U(x)'s$. Finally it also knows the flags each bank has. \\
\\
The banks do not learn anything about the number of transactions each account is involved in, or even if the account is an Orderer or a Beneficiary. The aggregator has no way to find $x$, it only knows $U(x)$\\
\\
Suggestions to improve the privacy of this process:
\begin{enumerate}
    \item Encrypt the flags. Q: Who holds the key, how does this affect the training step?
    \item Create $U(X,i)$ for each transaction $i$, this would tell the bank how many transactions each account is part of. (They should already know this information though.) It would stop the aggregator learning the number of transactions between each pair of accounts.
    \item Find a way to do the $U(x) \mapsto F(x)$ step without the aggregator seeing each $F_B$. Does anyone know if there are MPC protocols to do this? \\
    \\
    A relatively straightforward solution would be to do this step in a TEE that is hosted by the aggregator. Then the aggregator would only see the final matrix of flags, from which it can learn almost nothing. It has no way of associating any entry with a specific account or even bank. Unfortunately TEE's are out of scope for this challenge, but it is worth mentioning as a note. 
\end{enumerate}

==> discussion.tex <==
% !TEX root =Feather.tex

\section{Discussion}\label{sec::discussion}
 







==> phase2_plan.tex <==
% !TEX root =Feather.tex

\section{Phase-II technical report plan}\label{sec::pahse2plan}

\begin{itemize}
    \item Problem statement
    \item Solution overview 
    \item Justify how our sharing of only binary values for flags and string distances follows the principle of privacy by design. Line of reasoning:
    \begin{itemize}
        \item Data Minimisation - SWIFT already has a model to detect anomalous transactions but believes data from Banks can help improve. This information can be at account level (flags) or transaction level (whether information provided for the particular transaction matches the information at banks). So, sharing whether this information at account and transaction level looks normal or anomalous is necessary and to an extent sufficient for the objective at hand. 
        \item Data confidentiality - Securely compute the string match feature with PSI protocol and share the flag values with LDP
    \end{itemize}
    \item Threat model and assumptions 
    \item Empirical results and Key contributions
    \begin{itemize}
        \item How we are going to write this section massively depends on the numbers we get for the accuracy, privacy, performance trade-off.
    \end{itemize}
    \item Technical details - String Match Features
    \item Technical details - Flag Collection (Along with the Protection Game)
    \item Technical details - SecureBoost
    \item Discussion
    \begin{itemize}
        \item Parameter selection and how the solution could be improved (in terms of accuracy at some cost to privacy and performance)
         \item How the solution can extend to use cases beyond the one at hand
        \item Limitations and constraints enforced by the flower framework
        \item Anything else 
    \end{itemize}
    \item Summary
\end{itemize}


\section{Empirical Analysis required}

\begin{itemize}
    \item Accuracy of the centralised model 
    \begin{itemize}
        \item Plain XGBoost model with no privacy constraints applied
        \item {\bf Output form:} Single number 
        \item {\bf Main uncertainty}
        \begin{itemize}
            \item Feature selection - should it be the binarised flags or actual flags? Similar question for the string match features. 
            \item Parameter selection for XGBoost 
        \end{itemize}
    \end{itemize}

    \item Plots comparing the privacy and AUPRC trade-off 
    \begin{itemize}
        \item Privacy measured as epsilon of LDP in one plot and inference privacy in the other. 
        \item Need this for privacy mechanisms found using the game with and without DP constraints, as well as randomised response. Need at least 10 points for each.
        \item Every point in these plots is the accuracy of model trained on data with the corresponding privacy mechanism applied. So, must train 30*cross-validation*iteration models
        \item All XGBoost models - no requirement of FATE
        \item {\bf Output form:} Two plots with three lines each on them - one line per method to generate a privacy mechanism. X-axis: privacy measure, Y-axis: AUPRC
        \item {\bf Main uncertainty}
        \begin{itemize}
            \item Parameter selection for XGBoost and the game
            \item \sout{Need to modify code for matching the flag values in train and test data.} 
            \item Should we also add noise for the string match features?
        \end{itemize}
    \end{itemize}

    \item Accuracy and Performance Metrics for SecureBoost under three different privacy scenarios
    \begin{itemize}
        \item Train SecureBoost model on data with privacy mechanisms applied using three different parameter values (one set for differential privacy, one set for the game)
        \item {\bf Output form:} Table with Seven Columns (one for name and the six columns corresponding to three privacy scenarios defined with DP and Inference Privacy. Rows can correspond to AUPRC on test data, AUPRC on train data, the agreed performance and scaling metrics
        \item {\bf Main uncertainty}
        \begin{itemize}
            \item SecureBoost code not working Flower on large datasets - can try running with just FATE backend in the worst-case scenario
            \item Parameter selection for SecureBoost and the game
            \item Agree on the exact metrics for performance and scaling - challenge recommendations: [total execution time, computation time for each party, maximum memory usage for each party, communication cost for each party] for  Efficiency, and [change in execution time and computation/communication as number of partitions increases] for Scalability. 

        \end{itemize}
    \end{itemize}
    
\end{itemize}

==> summary.tex <==
% !TEX root =Feather.tex

\section{Conclusion}\label{sec::summary}
STARLIT proposes a means by which SWIFT and a number of banks may collaboratively train and deploy a machine learning model to detect anomalous transactions. It is expected that this collaborative model will be significantly more effective than a model trained on SWIFT data alone. STARLIT consists of a feature extraction phase followed by a training phase. In this way, STARLIT is applicable to use cases with a data distribution that is challenging for conventional federated learning algorithms. It is also modular in that each phase can be modified depending on differing use case requirements. In the feature extraction phase we provide details both for 1) how SWIFT and the banks may collaboratively augment SWIFT's dataset with a number of features related to name and address discrepancies, to cope with real-world inconsistencies such as typos or encoding differences and 2) how account flags from the ordering and beneficiary account's banks may be securely aggregated by a third party 'flag collector'. Following this feature extraction, we show how SWIFT and the flag collector may then participate in a secure two-party vertical federated learning protocol to train the final anomaly detection model. The protocol trains an XGBoost model, given that XGBoost is widely used and represents the state of the art for tabular data, but could be adapted for other models. STARLIT yields a  level of privacy, security, and performance that is applicable to real-world scenarios. Beyond the challenge use case, the STARLIT approach may be applicable to collaborative detection of malware via analysis of sensitive network traffic and host activity logs, or protecting consumers against push payment fraud.











